Galactic Bulge Preferred Over Dark Matter for the Galactic Center Gamma-Ray Excess

An anomalous gamma-ray excess emission has been found in Fermi Large Area Telescope data covering the centre of the Galaxy. Several theories have been proposed for this `Galactic Centre Excess'. They include self-annihilation of dark matter particles, an unresolved population of millisecond pulsars, an unresolved population of young pulsars, or a series of burst events. Here we report on a new analysis that exploits hydrodynamical modelling to register the position of interstellar gas associated with diffuse Galactic gamma-ray emission. We find evidence that the Galactic Centre Excess gamma rays are statistically better described by the stellar over-density in the Galactic bulge and the nuclear stellar bulge, rather than a spherical excess. Given its non-spherical nature, we argue that the Galactic Centre Excess is not a dark matter phenomenon but rather associated with the stellar population of the Galactic bulge and nuclear bulge.

==> GCE_NatureAstronomyAddendum.tex <==
\begin{addendum}




  
     
 \item  RMC was the recipient of an Australian Research Council Future Fellowship (FT110100108). We thank Dustin Lang for  making available code and data which helped with generating the  X-bulge template and both
 Shogo Nishiyama 
and Kazuki Yasui for providing the data for the Nuclear bulge template. 
We
acknowledge the use of public data and software from the  Fermi data archives (http://fermi.gsfc.nasa.gov/ssc/). Finally,
the authors would also like to  thank Felix Aharonian, Anthony M. Brown,   Francesca Calore, 
Jean-Marc Casandjian,
H. Thankful Cromartie, Seth Digel, Torsten En{\ss}lin, Manoj Kaplinghat,
Ken Freeman, Ortwin Gerhard, Oleg Gnedin, Xiaoyuan
Huang, Naomi McClure-Griffiths, David Nataf, Ben Roberts, Miles Winter, Richard Tuffs, and Gabrijela Zaharijas for enlightening discussions.

\item[Author contributions]  OM designed and performed the majority of the data analysis. OM also constructed the Fermi Bubbles, Sun, Moon, Inverse Compton and Loop I templates. 
%CG and BC performed the Poisson modelling of the X-bulge contribution and 
CG processed the WISE data. RMC suggested the link with the X-bulge. BC processed the hydrodynamical 3D map into annuli density maps. DP created the interpolated annuli density maps. CG and SH assisted with the PS modelling. BC and DP created the dust maps. MP created the three dimensional HI and CO maps.
All authors
  contributed to the interpretation of the results.  The text of the final manuscript was mainly written by OM and CG, but all authors did have some contribution.


 \item[Competing Interests] The authors declare that they have no
competing financial interests.

\end{addendum}

==> GCE_NatureAstronomyAffiliations.tex <==
\begin{affiliations}
 \item Center for Neutrino Physics, Department of Physics, Virginia Tech, Blacksburg, VA 24061, USA
 \item School of Physical and Chemical Sciences,  University of Canterbury,
 Christchurch 8140, New Zealand
 \item Research School of Astronomy and Astrophysics, Australian National University, Canberra, Australia
 \item Institute of Physics and Astronomy, University of Potsdam, 14476 Potsdam-Golm, Germany
\item DESY, Platanenallee 6, 15738 Zeuthen, Germany
\end{affiliations}

==> GCE_NatureAstronomyMethods.tex <==
\begin{methods} \label{Methods}

%\input{GCE_NatureAstronomyMethods.tex}



\subsubsection*{\\Observations}


We examined $\sim 7$ years of Fermi-LAT data\cite{FermiInstrument2009} (August 4, 2008$-$September 4, 2015) selecting  \textsc{Pass 8} \textsc{ULTRACLEANVETO} %\footnote{\url{http://fermi.gsfc.nasa.gov/ssc/data/analysis/documentation/
%Pass8_usage.html
%}} 
class events. The data was extracted from a square region of $15^{\circ}\times15^{\circ}$ centred at Galactic coordinates $(l,b) = (0,0)$ and made no distinction between \textit{Front} and \textit{Back} events. Furthermore, we restricted our analysis
to the 667 MeV to 158 GeV energy range and used the
P8R2$_{-}$ULTRACLEANVETO$_{-}$V6 instrument response functions. To avoid contamination from terrestrial gamma-rays, we used events with zenith angles smaller than 90$^{\circ}$. This work made use of the Fermi Science Tools \texttt{v10r0p5} software package.



Employing the \texttt{gtmktime} tool we selected the recommended data filters\\ (DATA$_{-}$QUAL$>$0)\&\&(LAT$_{-}$CONFIG==1). Spatial binning was performed with the \texttt{gtbin} utility with which we divided the LAT data into $150\times 150$ angular bins of size $0.1^{\circ}$ in a \texttt{CAR} sky projection.






%\newpage

%\subsubsection*{Methods}
\subsubsection*{Templates}
The Galactic diffuse gamma-rays resulting from the interaction of cosmic-ray electrons and protons with the interstellar gas and radiation field were modelled with a similar method used for the standard Galactic diffuse emission model\cite{Casandjian:andFermiLat2016}.
%as that used for the 3FGL catalogue\cite{3FGL}.
We fitted a linear combination of atomic and molecular hydrogen gas templates (Supplementary Fig.~\ref{fig:densities} and \ref{fig:dust_maps}),
 an inverse Compton (IC) 
 energy-dependent spatial template
  as obtained with GALPROP\cite{Galpropsupplementary}, specialized templates for the \textit{Sun} and the \textit{Moon}, an isotropic component (\texttt{iso$_{-}$P8R2$_{-}$ULTRACLEANVETO$_{-}$V6$_{-}$v06.txt}), and a model for the gamma-ray emission associated with Loop I (Supplementary Fig.~\ref{fig:LoopI}).


The atomic and molecular hydrogen gas column densities were each distributed within four Galactocentric annuli to account for the non-uniform cosmic-ray flux in the Galaxy. The construction of these templates is described in Supplementary Sec.~1.



\subsubsection*{Bin-by-Bin Analysis}
\label{sec:methods} 

Similar to other works\cite{Ajello2016,FermiGCE2017},  we employed a bin-by-bin analysis technique, in which we split the Fermi-LAT data into 19 logarithmically spaced energy bins. Within each energy bin we performed a separate maximum-likelihood fit\cite{3FGL} with the \textit{pyLikelihood} analysis tool.
%\footnote{\url{http://fermi.gsfc.nasa.gov/ssc/data/analysis/documentation/}}. 
The bin size was chosen to be larger than the LAT energy resolution, but narrow enough that the Galactic emission spectral components can be simply approximated by a power law model.
% (PL: $dN/dE = N_0 E^{-\alpha} $ with norm $N_0$ and slope $\alpha$) formulas with fixed slopes. 
% We note that this bin-by-bin method
% means a parametric form
%  of the spectrum of the sources does not have to be chosen prior to the fit.The bin-by-bin method also significantly decreases the number of iterations required to reach convergence for our large number of parameters.
%OM:Change in response to Referee2:
 We note that this bin-by-bin method enables us to evaluate the likelihood for a test source with an arbitrary spectral model and significantly reduces the CPU power required to reach convergence as only the flux normalization of the sources are free to vary during the fits.
%OM==================


Once the bin-by-bin method had converged, the inferred spectrum of each source was either fitted by a power law or an exponential cut-off model. % If spectral bins with $TS<1$ were present then larger bin widths were used.
%Only spectral bins which had TS$\ge 1$ were used.
%OM:Change in response to Referee2:
When energy bins had 
 $TS<1$ or $\Delta F_i/F_i>1$ they were combined with adjacent energy bins until $TS>1$ and $\Delta F_i/F_i<1$. 
% This
%allows bands with upper limits to be treated consistently
%with the other bands so as to not introduce a potential bias to the fits.
% In practice, two different sets of energy bin combinations were applied: In the case of the spectral analysis of the new point source candidates, we combined the 19 energy bins into 4 bins [0.66, 1.19], [1.19, 2.81], [2.81, 11.86] and [11.86, 158.11] GeV. While for the extended sources analysis, we only combined the 5 energy bins between 28.12 and 158.11 GeV in the nuclear bulge case and the last 6 energy bins between 21.08 and 158.11 GeV in the X-bulge case.
%OM==================

 The errors from the bin-by-bin fit were added in quadrature to the  errors caused by the uncertainties in the
effective area\cite{3FGL}. These effective area errors were taken to be $f_i^{\rm rel}$ times the predicted flux for bin $i$. Where $f_i^{\rm rel}$ is interpolated from the values given in ref.~\citenum{3FGL}.
The spectrum was modelled by an exponential cut-off if   
\begin{equation}
{\rm TS}_{\rm curvature}\equiv 2\left(\log {\cal L}(\mbox{exp.~cut-off})-\log
{\cal L}({\mbox{power~law}})\right)\ge 9
\end{equation}
where ${\cal L}(i)$ is the maximum likelihood value for model $i$.

\subsubsection*{Comparing Hydrodynamic and Interpolated Gas Templates}
%\label{subsec:ptsrcsearch}


Initially we fit the LAT data with a model comprised of the 3FGL\cite{3FGL}  point sources present in our region of interest plus four other spatially extended sources (HESS J1825-137, RX J1713.7-3946, W28 and W30) reported in the 3FGL\cite{3FGL}. The spatial templates used to model these extended sources correspond to Version 14.  

To identify the most suitable gas templates for our study, we performed a scan in which we evaluated the improvement of the likelihood fit to the region of interest when the gas maps used were the ones created with the interpolation method or the hydrodynamical method (see Supplementary Sec.~1 for details of their construction). Supplementary Fig.~\ref{fig:pohvsinterp} shows that the data preferred
 the hydrodynamical method.



During optimisation, the flux normalisation of the 3FGL sources were left free in each energy bin.
We also simultaneously fit the 13 diffuse components' (H{\small I} annuli, CO annuli, dust templates, Loop I, inverse Compton, and isotropic) normalisation but kept the \textit{Sun} and \textit{Moon} fluxes fixed to their nominal values.

\subsubsection*{Point Source Search}
\label{subsec:ptsrcsearch}

In order to check whether any additional point sources are required, we followed a methodology similar to that described in refs.~\citenum{2FGL} and~\citenum{3FGL}.
%and the \textit{Fermipy}\footnote{http://fermipy.readthedocs.io/en/latest/} method used in ref.~\citenum{FermiGCE2017}.
We started from our \textit{baseline} model, which consists of all 3FGL point sources in the region of interest, Loop I, an inverse Compton template predicted by GALPROP, the hydrodynamical based gas maps, the recommended isotropic emission map, and a model for the Sun and the Moon (see Supplementary Sec.~1). We examined the significance of a trial point source with a power-law spectrum, with a fixed slope of two, %$\alpha=2.0$ 
at the centre of each pixel. The outcome of this  was a residual TS map where the \texttt{gttsmap} utility was used for this step. %The TS at each pixel is computed as $\mbox{TS} = 2(\log\mathcal{L} (\mbox{source}) - \log \mathcal{L} (\mbox{no-source}))$, where $\mathcal{L}$ is the likelihood of the data given the model with or without a source present at a given grid position. 
In accordance with our bin-by-bin method, a residual TS map was computed for each energy bin and these were then added to get a total residual map for the full energy range.   


From the total residual TS map we generated a list of all the pixel clusters with TS values above the detection threshold that looked reasonably isolated under visual inspection ($\sim 0.5^{\circ}$ of angular separation). The coordinates of the source candidates were calculated as the average of adjacent pixel positions weighted by their respective TS values\cite{2FGL}. A more sophisticated technique would be to fit the TS map with a two dimensional parabola. But, we found our results were not sensitive to the small difference in position that this gave.
To avoid convergence issues, at each step we added
only the ten (or fewer if less were available) brightest seeds  to our model and reran the bin-by-bin analysis routine where {\em all\/} components $-$ including the new point sources $-$ were simultaneously fitted.
Only the seeds that were found to have a TS above the detection threshold from this step were allowed to stay in the model. Note that this is an iterative procedure that goes from bright sources to faint ones. This procedure was repeated seven times in our region of interest until no seeds were found or no more point source candidates passed the thresholding step. This made the method more robust against source confusion. 
%
%We did not use \textit{gtfindsrc} to refine the seeds' positions because it is based on an unbinned likelihood method\cite{2FGL}.
When doing a global analysis, as opposed to a bin-by-bin analysis, each new point source candidate has two parameters for the power law and two parameters for its position. In that case a $\mbox{TS} \geq 25$ (which corresponds to 4$\sigma$) is used as the detection condition\cite{mattox,3FGL}. However, since we used a bin-by-bin analysis with 19 energy bands in each of which  the point source amplitude was not allowed to take on a negative value. As shown in  Supplementary Sec.~2, we thus have a mixture distribution given by 
\begin{equation}
%p(\mbox{TS})=\frac{ \delta(\mbox{TS}) +\sum_{i=1}^{19} \binom{19}{i} \chi_{i+2}^2(\mbox{TS})}{ \sum _{i=0}^{19} \binom{19}{i}}\\
p({\rm TS})= 2^{-n}\left(\delta({\rm TS}) +\sum_{i=1}^{n} \binom{n}{i} \chi_{i+2}^2({\rm TS})\right)
\label{eq:pTS}
\end{equation}
where  $\delta$ is the Dirac delta function, $\binom{19}{i}$ is a binomial coefficient, and $\chi_{i+2}^2$ is a $\chi^2$ distribution with $i+2$ degrees of freedom.
To work out the number of  $\sigma$ of a detection we evaluate the equivalent p-value for a one new parameter case\cite{wilks}:
\begin{equation}
\mbox{Number of $\sigma$}\equiv \sqrt{\rm InverseCDF\left(\chi_1^2,{\rm CDF}\left[p(\mbox{TS}),\hat{{\rm TS}}\right]\right)}
\end{equation}
where CDF and InverseCDF are the cumulative distribution and inverse cumulative distribution respectively. The first argument of each of these functions is the distribution function and the second is the value the CDF or InverseCDF is evaluated at. The observed TS value is denoted by $\hat{\rm TS}$.
It follows that 
we use a threshold of  $\mbox{TS} \ge 41.8$ to correspond to a 4$\sigma$ detection.  

The total set of new point source candidates found in this work are displayed in Supplementary Fig.~\ref{fig:tsmaps} along with the TS residual map obtained in our last iteration. Although the model including all the new point sources is a much better representation of the region of interest, a few hot spots still remain. These are, however, found to be below the detection threshold of $\mbox{TS}\ge 41.8$ in the maximum likelihood step. As can be seen from  Supplementary Fig.~\ref{fig:tsmaps}, the X-bulge morphology is clearly visible in the residual TS values. Although, along the Galactic plane, in comparison to  Fig.~\ref{fig:X-bulge_correlation} 
%and Supplementary Fig.~\ref{fig:xbulge}, 
the X-bulge morphology is shifted to negative longitudes (a similar shift is seen in refs.~\citenum{Casandjian:andFermiLat2016}, \citenum{YangAharonian2016}, and \citenum{FermiGCE2017} with the use of different methods), this may be due to degeneracies between the X-bulge template and the amplitude of the 3FGL and new point sources  around $l=0,b=0$. A similar phenomenon can be seen in Figs.~1 and 2 of ref.~\citenum{GordonMacias2013}. The Poisson noise is also very large in this region and so the mismatch did not have much bearing on the fit.

To identify possible multi-wavelength counterparts to the gamma-ray sources we searched in the seed locations % $-$ 
within the 68\% containment of the point spread function  for one of our highest energy bands $\sim 0.1^\circ -$ around each source in the ATNF pulsar\cite{ATNF:catalog}, globular cluster\cite{GBC:catalog}, supernova remnant (SNR)\cite{Green:SNRcatalog} and the Roma-BZCAT blazar\cite{Massaro2009} catalogues for potential gamma-ray emitters. We found spatial overlaps for 18 of our 64 point source candidates (see Supplementary Table~1). Note that this does not preclude the possibility that the other 46 point source candidates are real sources since high extinction towards the GC makes it difficult to have very complete  multi-wavelength source catalogs.

%Comparing to the 1FIG catalogueue\cite{Ajello2016},  
%14 out of 43 of our new point source candidates coincide with new point source candidates in
%1FIG (see Supplementary Table 1). While 1FIG finds 21 new point sources.
%not present in the 3FGL catalogueue. 
%This is a reasonable overlap considering
%that we used
%84 months of PASS 8 data while 1FIG was constructed from 62 months
%of PASS 7 data. % and so it is to be expected that we would detect a larger
%number of new point sources. 
%Also, the method used by 1FIG was somewhat stricter in it's acceptance criteria\cite{FermiGCE2017}.
Our new point sources are compared to the 2FIG\cite{Ajelloetal:2017} in Supplementary Fig.~\ref{fig:ptsrcs_comparison}. As can be seen, there is a reasonable overlap considering that the two analyses used different diffuse galactic emission templates and that 2FIG was based on a wider energy range (0.3 to 500 GeV) and time interval (7.5 years). It is reassuring that the majority of new 2FIG sources that are not associated with one of our new point sources are on a hot spot of our TS map. The list of point sources found in this work are provided in Supplementary Table 1. 


 Including the 3FGL sources, we had a total of 109 point source candidates in our $\left|l\right|<=7.5^\circ$, $\left|b\right|<=7.5^\circ$ region of interest. This is compatible with the 127 point source candidates found by ref.~\citenum{FermiGCE2017} for a disk like region of interest with radius 10$^\circ$.



\subsubsection*{New Templates}

\subsection*{X-bulge:}

We followed a procedure based on the method described in ref.~\citenum{NessLang2016} applied to the WISE data.
% We used the 3.4 (W1) and 4.6 (W2) micron WISE data masking
% out the top and bottom 5\% of pixels based on W1$-$W2 color, as well as pixels with negative flux. 
% We then subtracted a best fit exponential disk model from W1 and W2 where the disk amplitude was allowed to be different for the W1 and W2 bands.
% \begin{multline}
% \mbox{bulge}\propto  \exp
% \left(
% 	-
% 	\left\{
% 		\left(
%         	\frac{  (b-b_0)\cos (\theta )+(l-l_0)\sin (\theta ) }{\beta}
%         \right)^2 
%     \right. 
% \right.
%     \\
% \left.
%     \left.
%     \vphantom{\frac{  (b-b_0)\cos (\theta )+(l-l_0)\sin (\theta ) }{\beta}}
%         +[(l-l_0)\cos (\theta ) -(b-b_0)\sin (\theta ) ]^2
% 	\right\}^{1/2}
%     /\alpha
% \right)
% \end{multline}
% where $\alpha=1.2$~{ kpc}, $\beta=0.35$, $l_0=-0.45^\circ$,  $b_0=0.11^\circ$, and $\theta=0.06^\circ$.
% We then performed a  50 pixel ($~1.7^\circ$) median filter of masked residuals (median of unmasked pixels)
% on both exponential subtracted maps.
To use this template in comparisons with the Fermi-LAT data, all pixels values below zero were set to zero in each median filtered exponential subtracted map and our template was then constructed by taking the average of the two resultant maps. The resulting template is displayed 
%Supplementary Fig.~\ref{fig:xbulge}.
 by the white contours in Fig.~\ref{fig:X-bulge_correlation}.

\subsection*{Boxy Bulge:}

We assumed the triaxial model for the Galactic bulge derived in ref.~\citenum{Freudenreich:1998}. This was obtained by fitting to COBE/DIRBE near-infrared ($1.25-4.9$~$\mu$m) data. We adopted the best-fitting model in that reference, which is \textit{Model S}. This consists on a $\sech^2$ function on the bar radial spatial profile. The template used in our analysis is shown in Supplementary Fig.~\ref{fig:Boxybulge}. 

\subsection*{Nuclear Bulge:}

 We used a map constructed from a near-infrared stellar density measurement of the central region of our Galaxy ($|l|\geq 3^\circ$ and $|b|\geq 1^\circ$) and subtracted a best fit Galactic disk component\cite{Nishiyama2015}. 
 In order to remove artificial sharp boundaries in the map induced by survey patches, all pixels below 15 stars/arcmin$^2$ were set to zero. The resulting template is displayed 
by the black contours in Fig.~\ref{fig:X-bulge_correlation}. 
% in Supplementary Fig.~\ref{fig:NBstars}.


\subsection*{Dark Matter:}

We modelled the potential annihilating dark matter signal in the GC as the square of an NFW density profile with an inner slope of 1.2, which had been shown to describe the GCE well in previous works\cite{%Goodenough2009gk
hooperlinden2011,
%AbazajianKaplinghat2012,GordonMacias2013,MaciasGordon2014,
Abazajian2014,Daylan:2014%,
%CaloreCholisWeniger2015,
%Ajello2016
%,FermiGCE2017
}.
% : 
% \begin{equation}
% \rho (r) = \frac{\rho_\odot}{ \left(\frac{r} { R_\odot}\right)^\gamma  \left(\frac{1 + r/R_s}{1 + R_\odot/R_s}\right)^{3-\gamma} }, 
% \end{equation}
% where $R_\odot$ is the Sun's distance from the GC, $\rho_\odot$ is the dark matter density at $R_\odot$, $R_s$ is the scale radius of the Galaxy's dark matter halo, and gamma is the profile slope. We use standard values for these parameters to $R_s = 23.1$ kpc, $R_\odot = 8.25$ kpc and $\rho_\odot = 0.36$ GeV/cm$^3$, $\gamma=1.2$ \cite{GordonMacias2013}. We found our results were not qualitatively changed if we instead used the canonical  $\gamma=1$ value.
%
The square of an NFW density profile 
 %(NFW$^2$)
is representative of a tentative annihilating dark matter signal in the GC. 
%Alternatively, it could also represent an unresolved population of Galactic bulge MSPs \cite{AbazajianKaplinghat2012,MaciasGordon2014,YuanZhang2014}.


\subsection*{Fermi Bubbles:}
%Recently, Acero et al.\cite{Casandjian:andFermiLat2016} performed a morphological study of these structures in the inner $20^{\circ}$ of the GC. They found that the boundaries of the Fermi bubbles are well described by 
As found by  Acero et al.\cite{Casandjian:andFermiLat2016}, we use
two catenary curves of the form $10.5^\circ \times (\cosh((l - 1^\circ)/10.5^\circ) - 1^\circ)$ and $8.7^\circ \times(\cosh((l+1.7^\circ)/8.7^\circ) - 1^\circ)$ for the Northern and the Southern bubbles, respectively. 


%\end{description}


%\newpage





\subsubsection*{Testing Extended Emission Templates}
\label{Sec:extendedemission}




%We first examined the case in which the set of new point sources (Supplementary Table~1) is not included in the model. 
We fitted the gamma-ray emission with our bin-by-bin method to derive fluxes that are independent of the choice of spectral model. Within each bin, the spectrum of the included point and extended sources were modelled as power laws with fixed spectral index of two. Due to the small size of the bins, our results were not sensitive to the precise spectral index  used.
In each energy bin, the amplitudes of all included
point sources and all included extended templates were simultaneously fit.
%In each energy bin, the amplitudes of all sources were simultaneously fitted.
%CG: changed above sentence back to its original as we can use it in arguing reviewer 3 did not read our article carefully.
This allowed us to effectively marginalise over the statistical uncertainties.
%in these other sources. 
Table~1 shows the steps we took to evaluate whether a template was significantly detected.
We started with the \textit{baseline} model and then evaluated the TS of each new template. We then added the template with the highest TS to our model and repeated the procedure with this appended to the Base model. We iterated through these steps until the highest TS-value of a new template was below our $4\sigma$ threshold.
For each new template there are  $n\times 19$ new parameters.The probability distribution is the same as equation~(\ref{eq:pTS}) except that 
the 19 should be replaced by $n\times 19$ and 
the $\chi^2_{i+2}$ should be replaced with $\chi^2_i$
as we are not fitting the positions of the template.  This is the same formula as in case 9 of ref.~\citenum{SelfLiang87}. For one new template being considered (i.e.\ 19 new parameters),  our
 $4\sigma$  detection threshold corresponded to $TS\ge 38.4$. 

% The top panels of Supplementary Fig.~\ref{fig:GCE_syst_uncert} show that if we used the interpolated gas maps without including any new point sources,
% we were able to reproduce the results of previous studies\cite{AbazajianKaplinghat2012,GordonMacias2013,MaciasGordon2014,Abazajian2014,Daylan:2014,CaloreCholisWeniger2015,Ajello2016,FermiGCE2017}, while the bottom panels show that once we used our new gas maps, included our new point sources and our new extended templates for the X-bulge and nuclear bulge, the fitted dark matter amplitude is negligible in every energy bin. The improvement of the likelihood for various combinations of templates is shown in Supplementary Table~1.

The contributions of the different components for our proposed model of the GCE are shown in Supplementary Fig.~\ref{fig:ptsrc_spectra}. 
The fractional residuals are shown in Supplementary Fig.~\ref{fig:Residuals}. As can be seen from the top left  panel, the X-bulge is needed even when the interpolated gas maps are used. Comparing the top and bottom right panels shows that the X-bulge morphology has been accounted for by our template.

%The values for our combined X-bulge and nuclear bulge spectrum are given in Supplementary Table~\ref{Xnbulgetab}. 

\subsubsection*{Molecular-Hydrogen-To-CO Conversion Factor}
Our inferred molecular-hydrogen-to-CO conversion factor ($X_{CO}$) is shown in Supplementary Table~\ref{X_CO}. As in ref.~\citenum{Casandjian:andFermiLat2016} we evaluated $X_{CO}$ using our $2$~GeV energy bin fit results. Our values are consistent with the results from all sky fits as can be seen from comparing to Fig.~25 of ref.~\citenum{ackermannajelloatwood2012}. Although our 8 to 10 kpc best fit $X_{CO}$ is somewhat larger than the all sky and high latitude\cite{Casandjian2015} measurements, it does also have large error bars and so is still consistent with the other measurements at about  2$\sigma$ or better level even when only statistical errors are accounted for. As in ref.~\citenum{ackermannajelloatwood2012}, our $X_{CO}$ values for the outer annuli were strongly biased because the model  under-fitted the data in the outer galaxy and so we do not report them.


We found most of our results were not sensitive to changing the number of annuli to five. This was done by splitting our first annuli into two annuli with radii 0 to 1.5 kpc and 1.5 to 3.5 kpc as in ref.~\citenum{FermiGCE2017}. However,  we got unrealistic $X_{CO}$ values for the innermost annuli in that case.  Therefore, we stuck to the four annuli case shown in Supplementary Fig.~\ref{fig:densities}. Note that we did not explicitly use the $X_{CO}$ values in performing our fits and
we are only quoting their inferred values to demonstrate the fitted amplitudes for our interstellar gas maps are reasonably consistent with previous results.


\subsubsection*{Systematic Errors}\label{subSec:systerrors}
Our analysis involved making choices for the spin temperature, the cosmic-ray source distribution, the 	 $E(B-V)$ reddening  map magnitude cut,  and also whether or not to include a template for the Fermi bubbles. We evaluate the associated systematic errors by seeing how the best fit exponential cutoff parameters change when different choices were made. To do this for the  spin temperature, we used $T_S=150$~K instead of $T_S=170$~K.  For the inverse Compton model we changed the cosmic ray source distribution from ``Lorimer'' to ``OBstars''\cite{ackermannajelloatwood2012} as this was found to have the greatest effect on the inverse Compton morphology.   We found changing other parameters for the inverse Compton model had negligible effects. The dust systematic error was evaluated by changing the    $E(B-V)$ reddening  map magnitude cut from 5 mag and above to 2 mag and above.  The Fermi bubbles systematic error was obtained by including the catenary template in the fit. The resulting systematic errors are given in Table~2. 

We also checked the sensitivity of our results to the background model and new point sources. As can be seen from Supplementary Table~\ref{Tab:syslikelihoods}, the Xbulge+nuclear bulge are still needed by the data when no new point sources are included, or when the interpolated gas maps are used, or when the 2FIG point sources are used. The NFW-squared template was still needed by the data, after the X-bulge and nuclear bulge were included, only in the case of the interpolated gas maps. 

To evaluate the impact that potential mismodeling of the Galactic plane could have in our main results we masked the inner $|b|<1^{\circ}$ of the region of interest (see Supplementary  Fig.~\ref{fig:PlaneMask}) and utilized a statistical procedure similar to that in Table~1. We used the \texttt{Composite2} tool within the Fermi Science Tools and performed a composite likelihood analysis of the unmasked region of interests simultaneously for each energy bin (this method was first used in the GC region in ref.~\citenum{Horiuchi2016}). We tied across the regions $b>1^{\circ}$ and $b<-1^{\circ}$ of the inner $15^{\circ}\times 15^{\circ}$ of the GC and constrained the normalization of all the extended templates to be the same throughout the two separate region of interests at each energy bin. The majority of the new point sources as well as the nuclear bulge template reside in the $|b|<1^{\circ}$ region, so this analysis pipeline considered the 22 new point sources outside the masked region, the X-bulge and the NFW-squared templates in an attempt to model the GCE. The results are shown in Supplementary Table~\ref{Tab:PlaneMask}. As it can be seen, the data still significantly favours an X-bulge template over a spherical template.

As an additional check, we also evaluated the correlation matrix around our best fit model. We found that the correlation coefficients between all extended components and our X-bulge and nuclear bulge templates were in the range $10^{-10}$ to $10^{-2}$ in all energy bins.
With such small correlations even
systematic biases in the templates several times larger than the statistical uncertainties would not substantially affect the fitted normalizations of the two bulge templates. Further sources of systematic errors may arise from the choices made in constructing the X-bulge and nuclear bulge templates. We will investigate these in future work.


% \subsubsection*{Determining the X-bulge Contribution to the Resolved MSPs}


% The 3FGL and new point sources may have contributions from a number of sources such as the X-bulge, the nuclear bulge, the Galactic disk, extragalactic sources, and some may be small scale corrections to the diffuse Galactic emission model
%\cite{Ajello2016,3FGL}.
% We modelled the probability of a point source being resolved in pixel $i$ as a Poisson distribution 
% with mean
% \[
% \mu_i=\mu_{\mbox{\tiny Xbulge}} \mbox{Xbulge} (l_i,b_i)+\mu_{\rm isotropic}+\mu_{\rm exp} {\rm e}^{-|b_i|/\beta}
% \]
% where Xbulge$(l_i,b_i)$ is the value of the X-bulge template at pixel $i$.
% To determine the values of $\mu_{\mbox{\tiny Xbulge}}$, $\mu_{\rm isotropic}$, $\mu_{\rm exp}$, and $\beta$, we maximized the likelihood which is given by
% \[
% {\cal L}=\prod_{i\in \mbox{point source}} \mu_i {\rm e}^{-\mu_i}\times\prod_{i\not\in\mbox{point source}} {\rm e}^{-\mu_i}
% \]
% where the products are over pixels with and without point sources. 
% The contribution of the X-bulge for a point source at pixel $i$ is given by $\mu_{\mbox{\tiny Xbulge}} \mbox{Xbulge} (l_i,b_i) / \mu_i$ and is listed in Supplementary Tables~\ref{tab:Sources_xbulge2} and \ref{tab:3fglSources_xbulge}.



% Over the
% entire region of interest, the X-bulge 
% contribution to the resolved point sources was $\sum_i\mu_{\mbox{\tiny Xbulge}} \mbox{Xbulge} (l_i,b_i) /\sum_i \mu_i=0.16\pm0.05 $. We can estimate the total number of point sources attributable to the X-bulge by multiplying this quantity with the total number of resolved point sources in our region of interest.
% The scale height, of the exponential disk, was found to be $\beta=(34\pm 6)$~pc which is compatible with the scale height of the nuclear stellar disk component of the nuclear bulge\cite{Nishiyama2015}.

\end{methods}


==> GCE_NatureAstronomy_Main_Text.tex <==
The main challenge in pinning down the properties of the Galactic Centre Excess (GCE) is the  modelling of diffuse Galactic emission from the interaction of cosmic rays with interstellar gas and radiation fields, by far the dominant source of gamma-rays in this region. The Fermi-Large Area Telescope (LAT) Collaboration designed a diffuse Galactic emission model based on a 
%model-fitting 
 template\cite{Casandjian:andFermiLat2016} approach that is optimized to single-out gamma-ray point sources.
 %(PSs)
 %in the data
 This  approach presupposes that the diffuse Galactic emission can be modelled as a linear combination of interstellar gas, inverse Compton %(IC) 
 maps, and several other diffuse components. Due to the limited kinematic resolution of gas tracers towards the Galactic Centre (GC), interstellar gas correlated gamma rays from the GC direction are  difficult to disentangle. Previous studies\cite{MaciasGordon2014,CaloreCholisWeniger2015,FermiGCE2017} utilized interstellar gas maps that were constructed with an interpolation approach that assumed circular motion of interstellar gas. This kinematic assumption provides for an estimate of the distance to a %given
 part of the interstellar gas. However, it is  well established that the Galaxy contains a central bar which causes non-circular motion of interstellar gas in its inner regions, so assuming circularity introduces a significant and avoidable bias to gamma-ray analyses of the GC region\cite{Pohl2008}. 

We use Fermi-LAT data accumulated between August 4, 2008 and September 4, 2015 in the $15^{\circ}\times15^{\circ}$ region around the GC. Hydrodynamical simulations\cite{Pohl2008}
that account for the  effects of the Galactic bar were used to better determine the diffuse Galactic gamma-ray emission.  
To  evaluate the impact that the choice of interstellar gas models have on our results, we also constructed atomic and molecular hydrogen gas maps using an interpolation approach that reproduced those used in most previous gamma-ray analyses of the GC. We split each into 4 concentric rings, each with its own normalization parameter.
Details of the model components and approach are provided in the Methods section.

Interstellar gas map templates constructed using the results of hydrodynamical simulations were found to be a better description of the diffuse gamma-ray data than the standard interpolation-based maps with a log likelihood ratio $\approx$ 1362. 
As we have additional data compared to that used to construct the Fermi-LAT 3FGL catalogue\cite{3FGL} and since we also use a different Galactic diffuse emission model, we searched for new point sources. We found 64
 candidates (each with significance $\ge 4\sigma$) in our region of interest 
 %(ROI)
 which are shown as green crosses in Fig.~\ref{fig:X-bulge_correlation}. We  found multi-wavelength counterparts for 18 of our 64 point source candidates. 
This is similar to the 3FGL catalogue\cite{3FGL}
where some $\sim 1/3$ of the point sources do not have a multi-wavelength associations, especially in the GC region where there is high extinction and the diffuse Galactic emission model is more likely to require corrections.
Given our point source candidates have high statistical significance, including them quantitatively affects our results; however, they do not qualitatively affect our conclusions (see the Systematic Errors subsection of the Methods).

%old location of fig 1

Our dark matter template for the GCE is modelled by the square of an Navarro-Frenk-White (NFW) template with an inner slope of 1.2. 
Note that 
gamma-ray observations of dwarf spheroidal galaxies are 
in tension with the  dark matter interpretation of the GCE, but, when all the uncertainties are accounted for, do not definitively rule  out such an interpretation\cite{Keeley2017}. Extended gamma-ray emission in the GC may also arise from unresolved sources such as millisecond pulsars (MSPs)\cite{AbazajianKaplinghat2012,MaciasGordon2014} or young pulsars\cite{OLeary2015}, both of which have GeV-peaked gamma-ray spectra. Studies have also shown detectable non-Poissonian features in photon statistics\cite{Lee_etal:2016,Bartes_etal:2016}. However, these may be due to defects in the Galactic emission model\cite{Horiuchi2016}.
The young pulsar hypothesis requires  recent star formation given the $\lsim$ few Myr $\gamma$-ray lifetimes of ordinary pulsars. Such star formation is absent from most of the bulge except in the $r \lsim 100$ pc nuclear region; a young pulsar explanation of the GCE thus requires that the bulge contain pulsars that are launched out of the nucleus. It has been claimed that this can be achieved   by the pulsar's natal kicks\cite{OLeary2015}. While MSPs can be generated  from old stellar populations\cite{Ploeg2017}. 


We thus also consider Galactic bulge stellar templates. Almost half the stars\cite{Portail2015} in the Galactic bulge are on orbits that contribute to the appearance (from the Earth) of an X-shaped over-concentration (the `X-bulge')\cite{Nataf2010}. This structure has been   revealed in an  analysis\cite{NessLang2016} of 3.4 and 4.6 micron data collected by the WISE telescope\cite{WISE:instrument}. However, ref.~\citenum{JooLeeChung2017} argued that the X-shape is a processing artefact. Our aim is \textit{not} to scrutinize what is the correct bulge template, but rather, to explore the bulge as an example astrophysical template for the GCE that is alternative to dark matter.
%
Using standard maximum-likelihood estimation with an X-bulge template based on the average of the 3.4 and 4.6 micron data, we find that the addition of our X-bulge template improves the fit to the gamma-ray data at about the $16.1\sigma$ level (see Table~1).
%This extends  earlier work\cite{Abazajian2015} which 
%used a WISE based template on a smaller region of interest.
 Note that we do not claim that the X-bulge provides a fit 16.1-sigma better than any other possible bulge stellar template. 
What we have done is evaluate how much the likelihood improved when an X-bulge was added relative to the likelihood without any new component being added to account for the GCE. 
 We also tried a boxy shaped bulge (see Methods section), and found that it improves the fit to the data at the 14.6$\sigma$ level. 
Importantly, the last row of Table I demonstrates that even when the boxy bulge stellar map is considered instead of the X-bulge, the dark matter template is still confidently ruled out as an explanation of GCE. As the X-bulge has a slightly higher $\sigma$ than the boxy bulge,  we used the X-bulge in the rest of the article. Similar, results would be obtained with the boxy bulge template.



A further  stellar component within the wider Galactic bulge is the so-called nuclear bulge.
This disky distribution of stars concentrated within $\sim 230$ pc radius of the Galactic nucleus has experienced on-going star formation over the life of the Galaxy and represents $\sim 10$\% of the overall bulge mass\cite{LaunhardtZylkaMezger2002}. 
To determine whether the nuclear bulge template 
improves the fit to the Fermi-LAT gamma-ray data, we used a map constructed from a near-infrared stellar density measurement\cite{Nishiyama2015} and found a $10\sigma$ improvement in the fit (see Table~1). In Fig.~\ref{fig:X-bulge_correlation} we show the residual gamma-ray map obtained after subtraction of our best-fit galactic diffuse emission and point sources model. 
%Note that the fitting already included the X-bulge and nuclear bulge as proxy templates. This is a method
%required to avoid biasing the determination of the contribution from new extended components, see for example Fig.~3 of ref.~\citenum{FermiGCE2017}.
As can be seen, the X-bulge and nuclear bulge are well traced by our residual gamma-ray maps. The correlation with the X-bulge is more evident away from the plane where the hard-to-model diffuse Galactic emission is no longer so dominant and the Poisson noise is much lower. We have performed a  $\pm 1^\circ$ masking of the plane, and found consistent results (see Methods section). 


Best-fit spectral parameters were found using $\chi^2$ fitting to the inferred flux points for the energy bins. Relative to a power-law spectrum, the preferred spectral model (at $3.5\sigma$ and $5.1 \sigma$ respectively) for both the X-bulge and nuclear bulge templates was a power law with an exponential cut-off ($dN/dE\propto E^{-\Gamma}\exp(-E/E_{\rm cut})$). The X-bulge had a spectral slope of $\Gamma=1.9\pm 0.1$, an energy cut-off $E_{\rm cut}=10\pm 5$ GeV and a luminosity $L=(4.5\pm 0.3)\times 10^{36}$ erg/s  for $E\ge 100$ MeV. Similarly, the fit for the nuclear bulge yielded $\Gamma=1.9\pm 0.1$, $E_{\rm cut}=13\pm 4$ GeV and $L=(3.3\pm 0.3)\times 10^{36}$ erg/s. Here and in the rest of the article 68\% confidence intervals are used for error bars and we adopted 8.25 kpc for the   distance to the GC. When the X-bulge and nuclear bulge spectra were combined  (see  Fig.~\ref{fig:X-bulge+NBstars_spectra}), we found a power law exponential  model was still preferred relative to a  power law ($dN/dE\propto E^{-\alpha} $) model  at 5.0$\sigma$. The best fit spectral parameters for this case  
are shown in  Table~2.
The combined X-bulge and nuclear bulge spectral parameters are compatible with previous estimates of the GCE based on templates of dark matter as well as resolved MSPs and globular clusters containing MSPs\cite{MaciasGordon2014}. 
 
When the X-bulge and nuclear bulge templates are included in the fit, we found that a squared NFW template with an inner slope of 1.2 was not significantly detected, see Table~1. 
 The 95\% upper limit on this component's luminosity was found to be  $5\times 10^{36}$~erg/s. 
The luminosity for an NFW-squared profile from our model baseline+NP+NFW, displayed in  
%in row 11 of 
Table~2, is
consistent with previous estimates\cite{MaciasGordon2014} and is about an order of magnitude larger than the limit we obtain when the X-bulge and nuclear bulge templates are included.
Similarly, a dark matter template based on the square of 
 an NFW profile with an inner slope of 1.0 was undetected.

% \begin{figure*}[!htbp]
% \begin{center}
% \begin{tabular}{cc}
% \centering
% \includegraphics[scale=0.4]{GCE_new_vs_old_analysis.pdf} &  \includegraphics[scale=0.4]{TS_GCE_no_new_ptsrcs.pdf}\\
% \includegraphics[scale=0.4]{GCE_new_ptsrcs_xbulge_NBstars.pdf} &  \includegraphics[scale=0.4]{TS_GCE_new_ptsrcs_xbulge_NBstars.pdf}
% \end{tabular}

% %\small
% \caption{
% {\bf   Comparison to  previous results.}
% In the top left panel the dark matter energy spectrum as extracted from the $15^\circ \times 15^\circ$ around the GC assuming he square of an NFW profile with an inner slope $\gamma=1.2$. In the top right panel the TS values (see Table~1) obtained at each energy bin for the dark matter source are shown. %The first row
% In the top panels  we used the interpolated gas maps and did not include any new point or extended sources. We found   a 
% %total $\mbox{TS}_{{\rm NFW}^2}=1220$  for the dark matter source. With 19 degrees of freedom, this  corresponds to 
% a 33 $\sigma$ detection of dark matter, consistent with previous studies. 
% Note that the Calore et al.\cite{CaloreCholisWeniger2015} and the Gordon \& Macias\cite{GordonMacias2013} results are for slightly different regions of interest and so their agreement with each other and the top panel results is only expected to be qualitative.
%  Bottom: our new analysis where the hydrodynamic gas maps, new point sources and new extended X-bulge and nuclear bulge templates are included. The significance of the dark matter model has reduced to 1.0$\sigma$.\
%  On the LHS, the boxes and error bars cover a 68\% confidence interval and the points show the best fit values. \label{fig:GCE_syst_uncert}}
% %\normalsize
% \end{center}
% \end{figure*}
%The top panels of  Fig.~\ref{fig:GCE_syst_uncert} show that if we used the interpolated gas maps without including any new point sources,
%we were able to reproduce the results of previous studies\cite{AbazajianKaplinghat2012,GordonMacias2013,CaloreCholisWeniger2015,Ajello2016,FermiGCE2017}, while the bottom panels show that once we used our new gas maps, included our new point sources and our new extended templates for the X-bulge and nuclear bulge, the fitted dark matter amplitude is negligible in every energy bin. The improvement of the likelihood for various combinations of templates is shown in  Table~1.


% \begin{table*}[!htbp]\caption{{\bf Summary of the Likelihood analysis results\label{Tab:likelihoods}}}
% \centering
% \begin{threeparttable}
% %\scriptsize 
% \begin{tabular}{llllcrc}
% %\toprule
% \hline\hline
% Base  & Source &  $\log(\mathcal{L}_{\rm Base})$  & $\log(\mathcal{L}_{{\rm Base}+{\rm  Source}})$  &  $\mbox{TS}_{\rm Source}$& $\sigma$ & Number of\\ 
%            &              &                                  &                         &                                               & & source parameters\\\hline
% baseline  & FB&     -172461.4          &   -172422.3    &  78 & 6.9 & 19\\ 
% baseline  & NFW-s &    -172461.4       &  -172265.3       & 392 & 18.4 &  19\\  
% baseline  & Boxy bulge& -172461.4         & -172238.7          &445 & 19.7   & 19\\
% baseline  & X-bulge& -172461.4         &  -172224.1         & 475&  20.5  & 19\\
% baseline  & NFW &    -172461.4         &  -172167.9        & 587  &23.0 &  19\\  
% baseline  & NB&   -172461.4         &  -171991.8    & 939  & 29.5 & 19\\
% baseline  & NP&     -172461.4          &   -169804.1    & 5315& 55.7  &  $64\times 19$\\\hline
% baseline$+$NP  & FB&     -169804.1    & -169773.6      &61&  5.8   & 19\\
% baseline$+$NP  & NB&     -169804.1  & -169697.2      &214  &  13.0 & 19\\
% baseline$+$NP  & Boxy bulge&     -169804.1  & -169663.7      &  281& 15.3 & 19\\
% baseline$+$NP  &NFW&     -169804.1   &   -169623.3         &  362& 17.6   & 19\\
% baseline$+$NP  & X-bulge&     -169804.1  &   -169616.2   &376 &  18.0  & 19\\
% \hline
% baseline$+$NP$+$X-bulge     &NFW & -169616.2    &-169568.4 & 96& 7.9 & 19 \\ 
% baseline$+$NP$+$X-bulge     & NB & -169616.2    & -169542.0 & 148&10.4& 19 \\ \hline
% baseline$+$NP$+$X-bulge$+$NB  & NFW& -169542.0         &-169531.0      & 22 & 2.4  & 19\\
% baseline$+$NP$+$X-bulge$+$NB  & FB& -169542.0         &-169525.5      & 33   & 3.5& 19\\ 
%  \hline
% baseline$+$NP$+$NB  & X-bulge&  -169697.2       &  -169542.0    & 310   & 16.1& 19\\
% baseline$+$NP$+$NB  & Boxy bulge&  -169697.2       &  -169566.0    &  262  & 14.6& 19\\ 
% baseline$+$NP$+$NFW  & X-bulge+NB&  -169623.3       &  -169531.0    & 185   & 10.8& $2\times 19$\\
% baseline$+$NP$+$NFW$+$NB     & X-bulge & -169598.9    & -169531.0 &136 &9.9& 19 \\
% baseline$+$NP$+$Boxy bulge$+$NB  & NFW& -169566.0         &-169553.3      & 25 & 2.7  & 19\\
% \hline\hline
% \end{tabular}
% \begin{tablenotes}
%       \item The \textit{baseline} model consists of all 3FGL point sources in the region of interest, Loop I, an IC template predicted by GALPROP, the hydrodynamic based gas maps, the recommended isotropic emission map, and a model for the Sun and the Moon.
%  Other model templates considered are: the 64 new point sources (NP), the square of a generalised NFW profile with an inner slope $\gamma=1.2$ or the square of a ``standard NFW'' (NFW-s) with inner slope $\gamma=1$, an infrared X-bulge and a Boxy bulge template tracing old stars in the Galactic bulge, 
%        a nuclear bulge (NB) template 
%       and a template accounting for the Fermi Bubbles (FB). 
%       The maximized likelihoods ($\mathcal{L}$) are given for the Base and Base$+$Source models and the significance of the new source is given by 
%        TS$_{\rm Source}\equiv 2(\log(\mathcal{L}_{{\rm Base}+{\rm  Source}}) - \log(\mathcal{L}_{\rm Base}))$. Note that for both likelihoods all parameters are maximized and so the $\mathcal{L}_{{\rm Base}+{\rm  Source}}$ will have additional parameters whose number is given in the last column of the table. 
%        The conversion between TS$_{\rm Source}$ and $\sigma$ is discussed in the Methods section.
%     \end{tablenotes}
% \end{threeparttable}
% \end{table*}


% \subsubsection*{Alternative Explanations}


% \subsection*{Fermi Bubbles: }
% \label{subsubsec:FermiBubbules}


% \begin{table*}[!htbp]
% \centering
% \caption{\bf Exponential cut-off best-fit parameters with statistical and systematic errors to the X-bulge + nuclear bulge}
% \begin{tabular}{ | r | r | r | r | r | r | r | r | r | }
% \hline
% 	\multicolumn{1}{|c|}{Parameter}& \multicolumn{1}{|c|}{Best fit} & \multicolumn{1}{|c|}{Statistical} & 
%     \multicolumn{5}{|c|}{Systematic Error} \\ \cline{4-8}
% 	   &  & \multicolumn{1}{|c|}{Error} & \multicolumn{1}{|c|}{Spin}& \multicolumn{1}{|c|}{Inverse} & \multicolumn{1}{|c|}{Dust} & \multicolumn{1}{|c|}{Fermi} &\multicolumn{1}{|c|}{Total}\\ %\hline
%         &  &  & \multicolumn{1}{|c|}{Temperature}      &  \multicolumn{1}{|c|}{Compton}  &      & \multicolumn{1}{|c|}{Bubbles}  &   \\ \hline 
% $\Gamma$      & 2.0      & 0.1         & 0.1        & 0.1  & 0\phantom{.0}  & 0.1 & 0.2 \\
% $E_{\rm cut}/$GeV & 13\phantom{.0}       & 5\phantom{.0}            & 1\phantom{.0}           & 3\phantom{.0}  & 1\phantom{.0}     & 2\phantom{.0}    & 4\phantom{.0}            \\
% $L/(10^{36}$erg$/$s$)$              & 6\phantom{.0}         & 1\phantom{.0}            & 1\phantom{.0}           & 1\phantom{.0}   & 0\phantom{.0}     & 0\phantom{.0}    & 1\phantom{.0}  \\
% \hline
% \end{tabular}
% \T
% \parbox[t]{0.8\textwidth}{\label{SysErr}
% The statistical errors  are 1$\sigma$. The total systematic error was obtained by adding in quadrature the individual systematic errors. %The total error was obtained by adding in quadrature the total systematic error and the statistical error. 
% Luminosities were computed for $E>100$ MeV.}
% \end{table*}

The Fermi Bubbles\cite{Fermi:LatBubbles,Su:etal} 
%(FB)  
are lobes that extend up to  $\sim 7$  kpc from the Galactic plane. Recently, 
%Acero et al.\cite{Casandjian:andFermiLat2016} performed a  study of them in the inner $20^{\circ}$ of the GC. They found that
The boundaries of the Fermi bubbles are described by two catenary curves\cite{Casandjian:andFermiLat2016}, see Methods section.  
However, the catenary  geometry does not match the
%X-shaped 
 excess we
see in our residual and TS maps in Fig.~\ref{fig:X-bulge_correlation} and Supplementary Fig.~\ref{fig:tsmaps}.  We found the addition of a catenary template did not qualitatively affect our results. As this template had a low TS value (see Table~1) we did not include it in our final results but rather treated its potential presence as a systematic effect (see Table~2, Methods section, and Supplementary Sec.~3).

% In ref.~\citenum{Fermi:LatBubbles}, the spectrum of the Fermi bubbles was determined
% from the residuals in the energy range between 0.7 GeV and 10 GeV. They examined an area near the southern edge of the Fermi bubbles
% ($-55^\circ < b < -40^\circ$ and $-15^\circ < l < 15^\circ$). A power-law fit
% in this region had a spectral index index $1.9\pm0.1$. In contrast, we found our X-bulge and nuclear bulge, for the same energy range, had a power-law fit with a %\textcolor{red}{significantly} 
% softer spectral index of $2.20 \pm 0.05$.
% Also, we estimate the X-bulge plus nuclear bulge has a solid angle of 0.03~sr, and therefore a luminosity per solid angle of  $(1.0\pm 0.1)\times10^{38}$~erg/s/sr. By contrast, the Fermi bubbles, for $|b|\ge 10^\circ$,  have a solid angle of about 0.7~sr and a luminosity\cite{Fermi:LatBubbles} per solid angle of $(6.3\pm 0.1)\times 10^{37}$~erg/s/sr. Even taking a wide range of systematic effects into account, the highest luminosity\cite{Fermi:LatBubbles} per solid angle  for the Fermi bubbles was only $8.6\times 10^{37}$~erg/s/sr. 

% Ref.~\citenum{FermiGCE2017} used a spectral decomposition technique to determine the low latitude Fermi bubble contribution. However, their residuals for their GCE show the characteristic X-shape in their Fig.~3. Also, they found the addition of their Fermi bubbles template did not remove the need for an extra template to explain the GCE. In summary, current spatial and spectral evidence seems to disfavour a Fermi-bubbles explanation for all of the X-bulge and nuclear bulge emission.

% \subsection*{\\Galactic Ridge Cosmic Rays:}
% \label{subsubsec:20cm}

% A recent study\cite{MaciasGordon2014} carried out a Fermi-LAT analysis of the Galactic  ridge region ($2^\circ \times 1^\circ$ around the GC) using templates obtained from measurements at other wavelengths. Either a 20-cm  map %\cite{Yusef-Zadeh2013} 
% or a HESS residuals
% %\cite{Aharonian:2006} 
% %CG removed above two refs to try accommodate referees request for more references to be added while still staying within the 20 refs limit.
% map was used with similar results. 
% The 20-cm template was based on  Green Bank Telescope continuum emission data  which measures non-thermal and thermal plasma distributions. %\cite{law2008}. 

% We found this map could be used to replace the nuclear bulge template with a similar level of significance and spectrum. Therefore there is systematic uncertainty surrounding the fractional contribution of cosmic rays to the nuclear bulge. Compatible ranges of cosmic ray contribution are consistent with current models\cite{MacGorCroProf2015}.



A comparison between the properties of our proposed X-bulge and nuclear bulge MSPs with other MSP populations can be obtained by comparing the MSP luminosity to stellar mass ratio. Note that this comparison assumes the ratio of MSP mass to stellar mass is constant across the different considered regions which will only be approximately correct. The stellar mass\cite{Bland-Hawthorn2016} of the Galactic bulge is $1.5 \times 10^{10}$ solar masses ($M_\odot$) and the nuclear bulge has a mass of $\sim 1.4 \times 10^9 \msun$. According to ref.~\citenum{Portail2015}, instantaneous stellar mass contributing to the appearance of the X-bulge over-density represents about 25\% of the Galactic bulge.
However, as can be seen by comparing 
%Supplementary Fig.~\ref{fig:xbulge}
our white contours in Fig.~\ref{fig:X-bulge_correlation}
 to Fig.~18 of ref.~\citenum{Portail2015},
the method they use to determine this contribution underestimates the X-bulge we extract from the WISE data as it eliminates the central regions of the X-bulge that we have included in our template. Therefore, we estimate our X-bulge has an instantaneous stellar mass $\gtrsim 4 \times 10^{9} M_\odot$.
From these data we infer a $E\ge  100$ MeV luminosity-to-mass (LtM) ratio of  $\lesssim 2 \times 10^{27}$ erg/s/$M_\odot$ for the combined X-bulge and nuclear bulge structure.
%
This is similar to the LtM ratio we infer from ref.~\citenum{Winter2016} for the MSP emission from the entire Milky Way of 
$\sim 2 \times 10^{27}$ erg/s/$M_\odot$ and  less than the
  $\sim 5 \times 10^{28}$ erg/s/$M_\odot$ for globular cluster 47 Tuc\cite{FermiGlobularClusters}
(which has an MSP-dominated $>$ 100 MeV luminosity of $(4.8\pm 1.1)\times 10^{34}$ erg/s
 and stellar mass of about $10^6 M_\odot$). 




% The upper limit derived from the NFW-squared template implies the rest of the bulge has a LtM ratio less than  $\sim 8\times 10^{26}$ erg/s/$M_\odot$.
% The region of the bulge outside the nucleus has experienced little star formation for many Gyr (and its stellar density is much lower than in globular clusters, limiting the potential for dynamical formation of close  stellar binaries).
% There are systematic differences between the stellar populations of the X and the bulge outside the X with stars in the X both higher in metallicity and likely systematically younger than other bulge stars, indeed, the spheroidal bulge population is likely one of the oldest in the Galaxy\cite{Bland-Hawthorn2016}. 
% Given this, a relatively low LtM for the region outside the X is thus not unexpected given its MSPs are expected to be older (therefore slower spinning and less luminous) than the X region MSPs and MSPs found elsewhere in the Galaxy.



We have shown that the X-bulge (or boxy bulge) plus the nuclear bulge provide a better fit than the dark matter explanation. We have not explicitly checked the burst model, but current implementations 
are highly model dependent and  fine-tuned\cite{Cholis2015}. Also, the young pulsar explanation is typically associated with spherically symmetric templates\cite{OLeary2015} and so also disfavoured compared to our MSP based X-bulge (or boxy bulge)$+$nuclear bulge explanation.
Therefore,
we have shown, in agreement with other recent results\cite{Bartels2017},
that the Galactic bulge stellar distribution is preferred over a spherically symmetric NFW-squared  excess template.

%Further observations will be needed to confirm that MSPs really are the sources of the GCE. One approach to do this will be to try and resolve the MSPs making up the Galactic and nuclear bulge. 
%It may be that many of the unassociated point sources in this region are already resolved MSPs and part of the GCE. 
%Radio observations will likely be needed to confirm if these point sources are pulsating. 
%Even if they are confirmed to be point sources, it will still 
%be necessary to obtain more resolved point sources from future observations to determine whether the Galactic bulge$+$nuclear bulge templates are being traced to a statistically significant extent.

 




==> GCE_NatureAstronomy_Main_refs.tex <==
\begin{thebibliography}{10}
\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
\providecommand{\bibinfo}[2]{#2}
\providecommand{\eprint}[2][]{\url{#2}}
\bibitem{FermiInstrument2009}
\bibinfo{author}{{Atwood}, W.~B.} \emph{et~al.}
\newblock \bibinfo{title}{{The Large Area Telescope on the Fermi Gamma-Ray
  Space Telescope Mission}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{697}},
  \bibinfo{pages}{1071--1102} (\bibinfo{year}{2009}).
\newblock \eprint{0902.1089}.

\bibitem{Goodenough2009gk}
\bibinfo{author}{{Goodenough}, L.} \& \bibinfo{author}{{Hooper}, D.}
\newblock \bibinfo{title}{{Possible Evidence For Dark Matter Annihilation In
  The Inner Milky Way From The Fermi Gamma Ray Space Telescope}}.
\newblock \emph{\bibinfo{journal}{ArXiv e-prints (arXiv:0910.2998)}}
  (\bibinfo{year}{2009}).
\newblock \eprint{0910.2998}.

\bibitem{FermiGCE2017}
\bibinfo{author}{{Ackermann}, M.} \emph{et~al.}
\newblock \bibinfo{title}{{The Fermi Galactic Center GeV Excess and
  Implications for Dark Matter}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{840}},
  \bibinfo{pages}{43} (\bibinfo{year}{2017}).
\newblock \eprint{1704.03910}.

\bibitem{CaloreCholisWeniger2015}
\bibinfo{author}{{Calore}, F.}, \bibinfo{author}{{Cholis}, I.} \&
  \bibinfo{author}{{Weniger}, C.}
\newblock \bibinfo{title}{{Background model systematics for the Fermi GeV
  excess}}.
\newblock \emph{\bibinfo{journal}{\jcap}} \textbf{\bibinfo{volume}{3}},
  \bibinfo{pages}{38} (\bibinfo{year}{2015}).
\newblock \eprint{1409.0042}.

\bibitem{AbazajianKaplinghat2012}
\bibinfo{author}{Abazajian, K.~N.} \& \bibinfo{author}{Kaplinghat, M.}
\newblock \bibinfo{title}{{Detection of a Gamma-Ray Source in the Galactic
  Center Consistent with Extended Emission from Dark Matter Annihilation and
  Concentrated Astrophysical Emission}}.
\newblock \emph{\bibinfo{journal}{\pr}} \textbf{\bibinfo{volume}{D86}},
  \bibinfo{pages}{083511} (\bibinfo{year}{2012}).
\newblock \eprint{1207.6047}.

\bibitem{OLeary2015}
\bibinfo{author}{{O'Leary}, R.~M.}, \bibinfo{author}{{Kistler}, M.~D.},
  \bibinfo{author}{{Kerr}, M.} \& \bibinfo{author}{{Dexter}, J.}
\newblock \bibinfo{title}{{Young Pulsars and the Galactic Center GeV Gamma-ray
  Excess}}.
\newblock \emph{\bibinfo{journal}{ArXiv e-prints (arXiv:1504.02477)}}
  (\bibinfo{year}{2015}).
\newblock \eprint{1504.02477}.

\bibitem{Cholis2015}
\bibinfo{author}{{Cholis}, I.} \emph{et~al.}
\newblock \bibinfo{title}{{The Galactic Center GeV excess from a series of
  leptonic cosmic-ray outbursts}}.
\newblock \emph{\bibinfo{journal}{\jcap}} \textbf{\bibinfo{volume}{12}},
  \bibinfo{pages}{005} (\bibinfo{year}{2015}).
\newblock \eprint{1506.05119}.

\bibitem{Casandjian:andFermiLat2016}
\bibinfo{author}{{Acero}, F.} \emph{et~al.}
\newblock \bibinfo{title}{{Development of the Model of Galactic Interstellar
  Emission for Standard Point-source Analysis of Fermi Large Area Telescope
  Data}}.
\newblock \emph{\bibinfo{journal}{Astrophys. J. Supp.}}
  \textbf{\bibinfo{volume}{223}}, \bibinfo{pages}{26} (\bibinfo{year}{2016}).
\newblock \eprint{1602.07246}.

\bibitem{MaciasGordon2014}
\bibinfo{author}{Macias, O.} \& \bibinfo{author}{Gordon, C.}
\newblock \bibinfo{title}{{Contribution of cosmic rays interacting with
  molecular clouds to the Galactic Center gamma-ray excess}}.
\newblock \emph{\bibinfo{journal}{Phys. Rev.}} \textbf{\bibinfo{volume}{D89}},
  \bibinfo{pages}{063515} (\bibinfo{year}{2014}).
\newblock \eprint{1312.6671}.

\bibitem{Pohl2008}
\bibinfo{author}{{Pohl}, M.}, \bibinfo{author}{{Englmaier}, P.} \&
  \bibinfo{author}{{Bissantz}, N.}
\newblock \bibinfo{title}{{Three-Dimensional Distribution of Molecular Gas in
  the Barred Milky Way}}.
\newblock \emph{\bibinfo{journal}{Astrophys.~J.}}
  \textbf{\bibinfo{volume}{677}}, \bibinfo{pages}{283--291}
  (\bibinfo{year}{2008}).
\newblock \eprint{0712.4264}.

\bibitem{3FGL}
\bibinfo{author}{{Acero}, F.}, \bibinfo{author}{{Ackermann}, M.},
  \bibinfo{author}{{Ajello}, M.}, \bibinfo{author}{{Albert}, A.} \emph{et~al.}
\newblock \bibinfo{title}{{Fermi Large Area Telescope Third Source Catalog}}.
\newblock \emph{\bibinfo{journal}{Astrophys. J. Supp.}}
  \textbf{\bibinfo{volume}{218}}, \bibinfo{pages}{23} (\bibinfo{year}{2015}).
\newblock \eprint{1501.02003}.

\bibitem{Keeley2017}
\bibinfo{author}{Keeley, R.}, \bibinfo{author}{Abazajian, K.},
  \bibinfo{author}{Kwa, A.}, \bibinfo{author}{Rodd, N.} \&
  \bibinfo{author}{Safdi, B.}
\newblock \bibinfo{title}{{What the Milky Way's Dwarfs tell us about the
  Galactic Center extended excess}}  (\bibinfo{year}{2017}).
  \newblock \emph{\bibinfo{journal}{ArXiv e-prints (arXiv:1710.03215)}}
  (\bibinfo{year}{2017}).
\newblock \eprint{1710.03215}.

\bibitem{Lee_etal:2016}
\bibinfo{author}{{Lee}, S.~K.}, \bibinfo{author}{{Lisanti}, M.},
  \bibinfo{author}{{Safdi}, B.~R.}, \bibinfo{author}{{Slatyer}, T.~R.} \&
  \bibinfo{author}{{Xue}, W.}
\newblock \bibinfo{title}{{Evidence for Unresolved {$\gamma$} -Ray Point
  Sources in the Inner Galaxy}}.
\newblock \emph{\bibinfo{journal}{\prl}} \textbf{\bibinfo{volume}{116}},
  \bibinfo{pages}{051103} (\bibinfo{year}{2016}).
\newblock \eprint{1506.05124}.

\bibitem{Bartes_etal:2016}
\bibinfo{author}{{Bartels}, R.}, \bibinfo{author}{{Krishnamurthy}, S.} \&
  \bibinfo{author}{{Weniger}, C.}
\newblock \bibinfo{title}{{Strong Support for the Millisecond Pulsar Origin of
  the Galactic Center GeV Excess}}.
\newblock \emph{\bibinfo{journal}{\prl}} \textbf{\bibinfo{volume}{116}},
  \bibinfo{pages}{051102} (\bibinfo{year}{2016}).
\newblock \eprint{1506.05104}.

\bibitem{Horiuchi2016}
\bibinfo{author}{Horiuchi, S.}, \bibinfo{author}{Kaplinghat, M.} \&
  \bibinfo{author}{Kwa, A.}
\newblock \bibinfo{title}{{Investigating the Uniformity of the Excess Gamma
  rays towards the Galactic Center Region}}.
\newblock \emph{\bibinfo{journal}{JCAP}} \textbf{\bibinfo{volume}{1611}},
  \bibinfo{pages}{053} (\bibinfo{year}{2016}).
\newblock \eprint{1604.01402}.

\bibitem{Ploeg2017}
\bibinfo{author}{Ploeg, H.}, \bibinfo{author}{Gordon, C.},
  \bibinfo{author}{Crocker, R.} \& \bibinfo{author}{Macias, O.}
\newblock \bibinfo{title}{{Consistency Between the Luminosity Function of
  Resolved Millisecond Pulsars and the Galactic Center Excess}}.
\newblock \emph{\bibinfo{journal}{JCAP}} \textbf{\bibinfo{volume}{1708}},
  \bibinfo{pages}{015} (\bibinfo{year}{2017}).
\newblock \eprint{1705.00806}.

\bibitem{Portail2015}
\bibinfo{author}{{Portail}, M.}, \bibinfo{author}{{Wegg}, C.} \&
  \bibinfo{author}{{Gerhard}, O.}
\newblock \bibinfo{title}{{Peanuts, brezels and bananas: food for thought on
  the orbital structure of the Galactic bulge}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{450}},
  \bibinfo{pages}{L66--L70} (\bibinfo{year}{2015}).
\newblock \eprint{1503.07203}.

\bibitem{Nataf2010}
\bibinfo{author}{{Nataf}, D.~M.}, \bibinfo{author}{{Udalski}, A.},
  \bibinfo{author}{{Gould}, A.}, \bibinfo{author}{{Fouqu{\'e}}, P.} \&
  \bibinfo{author}{{Stanek}, K.~Z.}
\newblock \bibinfo{title}{{The Split Red Clump of the Galactic Bulge from
  OGLE-III}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{721}},
  \bibinfo{pages}{L28--L32} (\bibinfo{year}{2010}).
\newblock \eprint{1007.5065}.

\bibitem{NessLang2016}
\bibinfo{author}{{Ness}, M.} \& \bibinfo{author}{{Lang}, D.}
\newblock \bibinfo{title}{{The X-shaped Bulge of the Milky Way Revealed by
  WISE}}.
\newblock \emph{\bibinfo{journal}{Astrophys.~J.}}
  \textbf{\bibinfo{volume}{152}}, \bibinfo{pages}{14} (\bibinfo{year}{2016}).
\newblock \eprint{1603.00026}.

\bibitem{WISE:instrument}
\bibinfo{author}{{Wright}, E.~L.} \emph{et~al.}
\newblock \bibinfo{title}{{The Wide-field Infrared Survey Explorer (WISE):
  Mission Description and Initial On-orbit Performance}}.
\newblock \emph{\bibinfo{journal}{Astrophys.~J.}}
  \textbf{\bibinfo{volume}{140}}, \bibinfo{pages}{1868--1881}
  (\bibinfo{year}{2010}).
\newblock \eprint{1008.0031}.

\bibitem{JooLeeChung2017}
\bibinfo{author}{{Joo}, S.-J.}, \bibinfo{author}{{Lee}, Y.-W.} \&
  \bibinfo{author}{{Chung}, C.}
\newblock \bibinfo{title}{{New Insight on the Origin of the Double Red Clump in
  the Milky Way Bulge}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{840}},
  \bibinfo{pages}{98} (\bibinfo{year}{2017}).
\newblock \eprint{1609.01294}.

\bibitem{LaunhardtZylkaMezger2002}
\bibinfo{author}{{Launhardt}, R.}, \bibinfo{author}{{Zylka}, R.} \&
  \bibinfo{author}{{Mezger}, P.~G.}
\newblock \bibinfo{title}{{The nuclear bulge of the Galaxy. III. Large-scale
  physical characteristics of stars and interstellar matter}}.
\newblock \emph{\bibinfo{journal}{\aap}} \textbf{\bibinfo{volume}{384}},
  \bibinfo{pages}{112--139} (\bibinfo{year}{2002}).
\newblock \eprint{astro-ph/0201294}.

\bibitem{Nishiyama2015}
\bibinfo{author}{Nishiyama, S.} \emph{et~al.}
\newblock \bibinfo{title}{Magnetically confined interstellar hot plasma in the
  nuclear bulge of our galaxy}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{769}},
  \bibinfo{pages}{L28} (\bibinfo{year}{2013}).
\newblock \urlprefix\url{http://stacks.iop.org/2041-8205/769/i=2/a=L28}.

\bibitem{Fermi:LatBubbles}
\bibinfo{author}{{Ackermann}, M.} \emph{et~al.}
\newblock \bibinfo{title}{{The Spectrum and Morphology of the Fermi Bubbles}}.
\newblock \emph{\bibinfo{journal}{Astrophys.~J.}}
  \textbf{\bibinfo{volume}{793}}, \bibinfo{pages}{64} (\bibinfo{year}{2014}).
\newblock \eprint{1407.7905}.

\bibitem{Su:etal}
\bibinfo{author}{{Su}, M.}, \bibinfo{author}{{Slatyer}, T.~R.} \&
  \bibinfo{author}{{Finkbeiner}, D.~P.}
\newblock \bibinfo{title}{{Giant Gamma-ray Bubbles from Fermi-LAT: Active
  Galactic Nucleus Activity or Bipolar Galactic Wind?}}
\newblock \emph{\bibinfo{journal}{Astrophys.~J.}}
  \textbf{\bibinfo{volume}{724}}, \bibinfo{pages}{1044--1082}
  (\bibinfo{year}{2010}).
\newblock \eprint{1005.5480}.

\bibitem{Bland-Hawthorn2016}
\bibinfo{author}{{Bland-Hawthorn}, J.} \& \bibinfo{author}{{Gerhard}, O.}
\newblock \bibinfo{title}{{The Galaxy in Context: Structural, Kinematic, and
  Integrated Properties}}.
\newblock \emph{\bibinfo{journal}{\araa}} \textbf{\bibinfo{volume}{54}},
  \bibinfo{pages}{529--596} (\bibinfo{year}{2016}).
\newblock \eprint{1602.07702}.

\bibitem{Winter2016}
\bibinfo{author}{Winter, M.}, \bibinfo{author}{Zaharijas, G.},
  \bibinfo{author}{Bechtol, K.} \& \bibinfo{author}{Vandenbroucke, J.}
\newblock \bibinfo{title}{{Estimating the GeV Emission of Millisecond Pulsars
  in Dwarf Spheroidal Galaxies}}.
\newblock \emph{\bibinfo{journal}{Astrophys. J.}}
  \textbf{\bibinfo{volume}{832}}, \bibinfo{pages}{L6} (\bibinfo{year}{2016}).
\newblock \eprint{1607.06390}.

\bibitem{FermiGlobularClusters}
\bibinfo{author}{{Abdo}, A.~A.} \emph{et~al.}
\newblock \bibinfo{title}{{A population of gamma-ray emitting globular clusters
  seen with the Fermi Large Area Telescope}}.
\newblock \emph{\bibinfo{journal}{\aap}} \textbf{\bibinfo{volume}{524}},
  \bibinfo{pages}{A75} (\bibinfo{year}{2010}).
\newblock \eprint{1003.3588}.

\bibitem{Bartels2017}
\bibinfo{author}{Bartels, R.}, \bibinfo{author}{Storm, E.},
  \bibinfo{author}{Weniger, C.} \& \bibinfo{author}{Calore, F.}
\newblock \bibinfo{title}{{The Fermi-LAT GeV Excess Traces Stellar Mass in the
  Galactic Bulge.}} 
  \newblock \emph{\bibinfo{journal}{ArXiv e-prints (arXiv:1711.04778)}}
  (\bibinfo{year}{2017}).
\newblock \eprint{1711.04778}.

\bibitem{Ajello2016}
\bibinfo{author}{Ajello, M.} \emph{et~al.}
\newblock \bibinfo{title}{{Fermi-LAT Observations of High-Energy $\gamma$-Ray
  Emission Toward the Galactic Center}}.
\newblock \emph{\bibinfo{journal}{Astrophys.~J.}}
  \textbf{\bibinfo{volume}{819}}, \bibinfo{pages}{44} (\bibinfo{year}{2016}).
\newblock \eprint{1511.02938}.



\end{thebibliography}



==> GCE_NatureAstronomy_Method_refs.tex <==
\begin{thebibliography}{10}
\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
\providecommand{\bibinfo}[2]{#2}
\providecommand{\eprint}[2][]{\url{#2}}
\makeatletter
\addtocounter{\@listctr}{30}
\makeatother

%\begin{thebibliography}{10}
%\expandafter\ifx\csname url\endcsname\relax
%  \def\url#1{\texttt{#1}}\fi
%\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
%\providecommand{\bibinfo}[2]{#2}
%\providecommand{\eprint}[2][]{\url{#2}}

\bibitem{Galpropsupplementary}
\bibinfo{author}{{Strong}, A.~W.} \emph{et~al.}
\newblock \bibinfo{title}{Galprop version 54: Explanatory supplement}.
\newblock \bibinfo{howpublished}{\url{http://galprop.stanford.edu}}.
\newblock \bibinfo{note}{Accessed: 2014-02-20}.

\bibitem{2FGL}
\bibinfo{author}{Nolan, P.~L.} \emph{et~al.}
\newblock \bibinfo{title}{{Fermi Large Area Telescope Second Source Catalog}}.
\newblock \emph{\bibinfo{journal}{Astrophys. J. Supp.}}
  \textbf{\bibinfo{volume}{199}}, \bibinfo{pages}{31} (\bibinfo{year}{2012}).
\newblock \eprint{1108.1435}.

\bibitem{mattox}
\bibinfo{author}{Mattox, J.} \emph{et~al.}
\newblock \bibinfo{title}{{The Likelihood Analysis of EGRET Data}}.
\newblock \emph{\bibinfo{journal}{Astrophys. J.}}
  \textbf{\bibinfo{volume}{461}}, \bibinfo{pages}{396} (\bibinfo{year}{1996}).

\bibitem{wilks}
\bibinfo{author}{Wilks, S.~S.}
\newblock \bibinfo{title}{{The Large-Sample Distribution of the Likelihood
  Ratio for Testing Composite Hypotheses}}.
\newblock \emph{\bibinfo{journal}{Ann.~Math.~Stat.}}
  \textbf{\bibinfo{volume}{9}}, \bibinfo{pages}{60} (\bibinfo{year}{1938}).

\bibitem{YangAharonian2016}
\bibinfo{author}{{Yang}, R.-Z.} \& \bibinfo{author}{{Aharonian}, F.}
\newblock \bibinfo{title}{{On the GeV excess in the diffuse {$\gamma$}-ray
  emission towards the Galactic centre}}.
\newblock \emph{\bibinfo{journal}{\aap}} \textbf{\bibinfo{volume}{589}},
  \bibinfo{pages}{A117} (\bibinfo{year}{2016}).
\newblock \eprint{1602.06764}.

\bibitem{GordonMacias2013}
\bibinfo{author}{Gordon, C.} \& \bibinfo{author}{Macias, O.}
\newblock \bibinfo{title}{{Dark Matter and Pulsar Model Constraints from
  Galactic Center Fermi-LAT Gamma Ray Observations}}.
\newblock \emph{\bibinfo{journal}{\pr}} \textbf{\bibinfo{volume}{D88}},
  \bibinfo{pages}{083521} (\bibinfo{year}{2013}).
\newblock \eprint{1306.5725}.

\bibitem{ATNF:catalog}
\bibinfo{author}{{Manchester}, R.~N.}, \bibinfo{author}{{Hobbs}, G.~B.},
  \bibinfo{author}{{Teoh}, A.} \& \bibinfo{author}{{Hobbs}, M.}
\newblock \bibinfo{title}{{The Australia Telescope National Facility Pulsar
  Catalogue}}.
\newblock \emph{\bibinfo{journal}{\aj}} \textbf{\bibinfo{volume}{129}},
  \bibinfo{pages}{1993--2006} (\bibinfo{year}{2005}).
\newblock \eprint{astro-ph/0412641}.

\bibitem{GBC:catalog}
\bibinfo{author}{{Harris}, W.~E.}
\newblock \bibinfo{title}{{A Catalog of Parameters for Globular Clusters in the
  Milky Way}}.
\newblock \emph{\bibinfo{journal}{\aj}} \textbf{\bibinfo{volume}{112}},
  \bibinfo{pages}{1487} (\bibinfo{year}{1996}).

\bibitem{Green:SNRcatalog}
\bibinfo{author}{{Green}, D.~A.}
\newblock \bibinfo{title}{{A catalogue of 294 Galactic supernova remnants}}.
\newblock \emph{\bibinfo{journal}{\basi}} \textbf{\bibinfo{volume}{42}},
  \bibinfo{pages}{47--58} (\bibinfo{year}{2014}).
\newblock \eprint{1409.0637}.

\bibitem{Massaro2009}
\bibinfo{author}{{Massaro}, E.} \emph{et~al.}
\newblock \bibinfo{title}{{Roma-BZCAT: a multifrequency catalogue of blazars}}.
\newblock \emph{\bibinfo{journal}{\aap}} \textbf{\bibinfo{volume}{495}},
  \bibinfo{pages}{691--696} (\bibinfo{year}{2009}).
\newblock \eprint{0810.2206}.

\bibitem{Ajelloetal:2017}
\bibinfo{author}{{Fermi-LAT Collaboration}}.
\newblock \bibinfo{title}{{Characterizing the population of pulsars in the
  Galactic bulge with the $Fermi$ Large Area Telescope}}.
\newblock \emph{\bibinfo{journal}{ArXiv e-prints}}  (\bibinfo{year}{2017}).
\newblock \eprint{1705.00009}.

\bibitem{Freudenreich:1998}
\bibinfo{author}{{Freudenreich}, H.~T.}
\newblock \bibinfo{title}{{A COBE Model of the Galactic Bar and Disk}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{492}},
  \bibinfo{pages}{495--510} (\bibinfo{year}{1998}).
\newblock \eprint{astro-ph/9707340}.

\bibitem{hooperlinden2011}
\bibinfo{author}{Hooper, D.} \& \bibinfo{author}{Linden, T.}
\newblock \bibinfo{title}{{On The Origin Of The Gamma Rays From The Galactic
  Center}}.
\newblock \emph{\bibinfo{journal}{\pr}} \textbf{\bibinfo{volume}{D84}},
  \bibinfo{pages}{123005} (\bibinfo{year}{2011}).
\newblock \eprint{1110.0006}.

\bibitem{Abazajian2014}
\bibinfo{author}{Abazajian, K.~N.}, \bibinfo{author}{Canac, N.},
  \bibinfo{author}{Horiuchi, S.} \& \bibinfo{author}{Kaplinghat, M.}
\newblock \bibinfo{title}{{Astrophysical and Dark Matter Interpretations of
  Extended Gamma-Ray Emission from the Galactic Center}}.
\newblock \emph{\bibinfo{journal}{Phys. Rev.}} \textbf{\bibinfo{volume}{D90}},
  \bibinfo{pages}{023526} (\bibinfo{year}{2014}).
\newblock \eprint{1402.4090}.

\bibitem{Daylan:2014}
\bibinfo{author}{Daylan, T.} \emph{et~al.}
\newblock \bibinfo{title}{{The characterization of the gamma-ray signal from
  the central Milky Way: A case for annihilating dark matter}}.
\newblock \emph{\bibinfo{journal}{Phys. Dark Univ.}}
  \textbf{\bibinfo{volume}{12}}, \bibinfo{pages}{1--23} (\bibinfo{year}{2016}).
\newblock \eprint{1402.6703}.

\bibitem{SelfLiang87}
\bibinfo{author}{Self, S.~G.} \& \bibinfo{author}{Liang, K.-Y.}
\newblock \bibinfo{title}{Asymptotic properties of maximum likelihood
  estimators and likelihood ratio tests under nonstandard conditions}.
\newblock \emph{\bibinfo{journal}{Journal of the American Statistical
  Association}} \textbf{\bibinfo{volume}{82}}, \bibinfo{pages}{605--610}
  (\bibinfo{year}{1987}).

\bibitem{ackermannajelloatwood2012}
\bibinfo{author}{Ackermann, M.} \emph{et~al.}
\newblock \bibinfo{title}{Fermi-lat observations of the diffuse gamma-ray
  emission: Implications for cosmic rays and the interstellar medium}.
\newblock \emph{\bibinfo{journal}{Astrophys. J.}}
  \textbf{\bibinfo{volume}{750}}, \bibinfo{pages}{3} (\bibinfo{year}{2012}).
\newblock \urlprefix\url{http://stacks.iop.org/0004-637X/750/i=1/a=3}.

\bibitem{Casandjian2015}
\bibinfo{author}{{Casandjian}, J.-M.}
\newblock \bibinfo{title}{{Local H i Emissivity Measured with Fermi-LAT and
  Implications for Cosmic-Ray Spectra}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{806}},
  \bibinfo{pages}{240} (\bibinfo{year}{2015}).
\newblock \eprint{1506.00047}.

\bibitem{kalberla2005}
\bibinfo{author}{{Kalberla}, P.~M.~W.} \emph{et~al.}
\newblock \bibinfo{title}{{The Leiden/Argentine/Bonn (LAB) Survey of Galactic
  HI. Final data release of the combined LDS and IAR surveys with improved
  stray-radiation corrections}}.
\newblock \emph{\bibinfo{journal}{\aap}} \textbf{\bibinfo{volume}{440}},
  \bibinfo{pages}{775--782} (\bibinfo{year}{2005}).
\newblock \eprint{astro-ph/0504140}.

\bibitem{dame2001}
\bibinfo{author}{{Dame}, T.~M.}, \bibinfo{author}{{Hartmann}, D.} \&
  \bibinfo{author}{{Thaddeus}, P.}
\newblock \bibinfo{title}{{The Milky Way in Molecular Clouds: A New Complete CO
  Survey}}.
\newblock \emph{\bibinfo{journal}{Astrophys.~J.}}
  \textbf{\bibinfo{volume}{547}}, \bibinfo{pages}{792--813}
  (\bibinfo{year}{2001}).
\newblock \eprint{astro-ph/0009217}.

\bibitem{Timur2011}
\bibinfo{author}{Delahaye, T.}, \bibinfo{author}{Fiasson, A.},
  \bibinfo{author}{Pohl, M.} \& \bibinfo{author}{Salati, P.}
\newblock \bibinfo{title}{{The GeV-TeV Galactic gamma-ray diffuse emission I.
  Uncertainties in the predictions of the hadronic component}}.
\newblock \emph{\bibinfo{journal}{Astron. Astrophys.}}
  \textbf{\bibinfo{volume}{531}}, \bibinfo{pages}{A37} (\bibinfo{year}{2011}).
\newblock \eprint{1102.0744}.

\bibitem{schlegel1998}
\bibinfo{author}{{Schlegel}, D.~J.}, \bibinfo{author}{{Finkbeiner}, D.~P.} \&
  \bibinfo{author}{{Davis}, M.}
\newblock \bibinfo{title}{{Maps of Dust Infrared Emission for Use in Estimation
  of Reddening and Cosmic Microwave Background Radiation Foregrounds}}.
\newblock \emph{\bibinfo{journal}{Astrophys.~J.}}
  \textbf{\bibinfo{volume}{500}}, \bibinfo{pages}{525--553}
  (\bibinfo{year}{1998}).
\newblock \eprint{astro-ph/9710327}.

\bibitem{Wolleben:2007}
\bibinfo{author}{{Wolleben}, M.}
\newblock \bibinfo{title}{{A New Model for the Loop I (North Polar Spur)
  Region}}.
\newblock \emph{\bibinfo{journal}{Astrophys.~J.}}
  \textbf{\bibinfo{volume}{664}}, \bibinfo{pages}{349--356}
  (\bibinfo{year}{2007}).
\newblock \eprint{0704.0276}.

\bibitem{gtsuntemp}
\bibinfo{author}{{Johannesson}, G.}, \bibinfo{author}{{Orlando}, E.} \&
  \bibinfo{author}{{for the Fermi-LAT collaboration}}.
\newblock \bibinfo{title}{{Accounting for the Sun and the Moon in Fermi-LAT
  Analysis}}.
\newblock \emph{\bibinfo{journal}{ArXiv e-prints (arXiv:1307.0197)}}
  (\bibinfo{year}{2013}).
\newblock \eprint{1307.0197}.

\bibitem{Chernoff1954}
\bibinfo{author}{Chernoff, H.}
\newblock \bibinfo{title}{{On the Distribution of the Likelihood Ratio}}.
\newblock \emph{\bibinfo{journal}{The Annals of Mathematical Statistics}}
  \textbf{\bibinfo{volume}{25}}, \bibinfo{pages}{573--578}
  (\bibinfo{year}{1954}).
\newblock
  \urlprefix\url{http://links.jstor.org/sici?sici=0003-4851\%28195409\%2925\%3A3\%3C573\%3AOTDOTL\%3E2.0.CO\%3B2-P}.

\bibitem{FermiInstrument}
\bibinfo{author}{Ackermann, M.} \emph{et~al.}
\newblock \bibinfo{title}{{The Fermi Large Area Telescope On Orbit: Event
  Classification, Instrument Response Functions, and Calibration}}.
\newblock \emph{\bibinfo{journal}{Astrophys. J. Supp.}}
  \textbf{\bibinfo{volume}{203}}, \bibinfo{pages}{4} (\bibinfo{year}{2012}).
\newblock \eprint{1206.1896}.


\end{thebibliography}

==> GCE_NatureAstronomy_abstract.tex <==
\textbf{An anomalous gamma-ray excess emission has been found in Fermi Large Area Telescope %(LAT)
data\cite{FermiInstrument2009} covering the centre of the Galaxy\cite{Goodenough2009gk,
%,AbazajianKaplinghat2012,GordonMacias2013,CaloreCholisWeniger2015,Ajello2016,
FermiGCE2017}. 
Several theories have been proposed for this `Galactic Centre Excess'.
%(GCE). 
They include self-annihilation of dark matter particles\cite{%Goodenough2009gk,AbazajianKaplinghat2012,GordonMacias2013,
CaloreCholisWeniger2015%,Ajello2016
}, an unresolved population of millisecond pulsars\cite{AbazajianKaplinghat2012
%,GordonMacias2013
}, an unresolved population of young pulsars\cite{OLeary2015}, or a series of burst events\cite{Cholis2015}. Here we report on a new analysis that exploits hydrodynamical modelling to register the position of interstellar gas associated with diffuse Galactic gamma-ray emission. We find evidence that the Galactic Centre Excess gamma rays are statistically better described by the  stellar over-density in the Galactic bulge and the nuclear stellar bulge, rather than a spherical excess. Given its non-spherical nature, we argue that the Galactic Centre Excess is not a dark matter phenomenon but rather associated with the stellar population of the Galactic bulge and nuclear bulge. }


==> figure_legends.tex <==
%\onecolumn
\begin{figure*}
% \centering
\centerline{
%\includegraphics[width=1.0\linewidth,trim=4pt 10pt 5pt 5pt, clip=false]{Fractionalresiduals_Xbulge+NBstars.pdf}
}
\caption
{
\textbf{Residual map of the \boldmath$15^\circ \times 15^\circ$ region of interest for $E \ge 667$ MeV}. The residuals are obtained as $(\mbox{Data} - \mbox{Model})$, where the model
includes 
 previously-detected 3FGL point sources (cyan squares)\cite{3FGL}, 64 additional point source candidates (green crosses) and
 the standard diffuse Galactic emission components related to the interstellar gas and radiation field. 
 %In order to not biasing the fit (see text), the model also included proxy templates for the X-bulge and nuclear bulge, which are added back to the residuals after the fit. 
 The white contours 
are the best-fit model counts from the X-bulge map obtained from analyses of WISE\cite{NessLang2016} infrared data after convolution the Fermi-LAT instrument response function.
The addition of a template based on the X-bulge 
 significantly improved the model fit to the gamma-ray data. 
 %at the  16$\sigma$ level. 
The cluster of point sources on the Galactic plane at 
 $l\approx6^\circ$ may be associated with the W28 (white dashed circle) supernova remnant\cite{Ajello2016,3FGL}. The zoomed-in region on the right shows the correlation with the near-infrared stellar density nuclear bulge data\cite{Nishiyama2015}, the black contours display the best-fit model counts associated with this component after convolution with the Fermi-LAT instrument response function. 
The X-bulge and nuclear bulge templates were included when the best fit parameters for the above model were found, but not when evaluating the above residuals.  A Gaussian with radius 0.3$^\circ$ was used to smooth the images and the upper limit of the colour scale has also been clipped for display purposes.
 \label{fig:X-bulge_correlation}}
\end{figure*}


\begin{figure}
\centering
%\begin{tabular}{c}
%\centering
\centerline{
%\includegraphics[width=1\linewidth,trim=4pt 10pt 5pt 5pt, clip=false ]{spectra_NBstars+Xbulge+NP_combined.pdf}
}
%\end{tabular}
\caption
{%\small 
\textbf{Differential flux of the new, statistically significant components in the Galactic Centre. }
The black boxes are the combined spectrum of the 64 new point source candidates, red boxes are the superposition of the nuclear bulge and X-bulge differential fluxes, while the green boxes display the sum of these three components and are compatible with previous results\cite{MaciasGordon2014,CaloreCholisWeniger2015},
although, the comparison should only be taken as qualitative as the previous results are for slightly different region of interest.
The box sizes encompass the 68\% confidence intervals. We found the combined nuclear bulge and X-bulge spectrum prefers an exponential cut-off to a power law model at 5$\sigma$. 
\label{fig:X-bulge+NBstars_spectra}}
\end{figure}
